Towards Explainable Student Group Collaboration Assessment Models Using Temporal Representations of Individual Student Roles

Collaboration is identified as a required and necessary skill for students to be successful in the fields of Science, Technology, Engineering and Mathematics (STEM). However, due to growing student population and limited teaching staff it is difficult for teachers to provide constructive feedback and instill collaborative skills using instructional methods. Development of simple and easily explainable machine-learning-based automated systems can help address this problem. Improving upon our previous work, in this paper we propose using simple temporal-CNN deep-learning models to assess student group collaboration that take in temporal representations of individual student roles as input. We check the applicability of dynamically changing feature representations for student group collaboration assessment and how they impact the overall performance. We also use Grad-CAM visualizations to better understand and interpret the important temporal indices that led to the deep-learning model's decision.

==> Related-Work.tex <==
\section{Related Work}\label{section_related-work}

There have been several recent works that explore using machine-learning concepts for collaboration problem-solving, analysis and assessment. For example, Reilly \emph{et al.} used Coh-Metrix indices (a natural language processing tool to measure cohesion for written/spoken texts) to train machine-learning models to classify co-located participant discourse in a multi-modal learning analytics study  \cite{reilly2019predicting}. Their multi-modal dataset contained eye-tracking, physiological and motion sensing data. Their study only had two collaboration quality states and focused on evaluating the level of cooperation between novice programmers that were instructed to program a robot. Using the same dataset, Huang \emph{et al.} used an unsupervised machine learning approach to discover unproductive collaborative states \cite{huang2019identifying}. They were able to develop a three-state solution that showed high correlation with task performance, collaboration quality and learning gain. Kang \emph{et al.} also used an unsupervised learning approach to study the collaborative problem-solving process of middle school students \cite{kang2019collaborative}. They analyzed data collected using a computer-based learning environment of student groups playing a serious game. For their analysis they employed \emph{KmL}, an R package for applying $k$-means clustering on longitudinal data \cite{genolini2011kml}. They too identified three different states using the proposed unsupervised method. In our paper we define five different group collaboration quality states in a supervised learning setup. 

Other prior works include - Talavera and Gaudioso utilized clustering methods to discover and characterize similar user behaviors in unstructured collaboration spaces \cite{talavera2004mining}. Spikol \emph{et al.} suggested using tools from multimodal learning analytics (MMLA) to gain insights into what happens when students are engaged in collaborative, project-based learning activities \cite{spikol2017using}. Soller \emph{et al.} proposed using Hidden Markov Models (HMM) to analyze and understand how group members in an on-line knowledge sharing conversation share, assimilate and build knowledge together \cite{soller2002machine}. Anaya and Boticario  explored unsupervised and supervised approaches to evaluate 12 quantitative statistical indicators of student interactions in a forum \cite{anaya2011application}. However, as mentioned by them, their proposed indicators do not have any semantic information of the message contents. For on-line collaborative tasks, Vrzakova \emph{et al.} examined unimodal data recordings (like screen activity, speech and body movements) and respective multimodal combinations, and tried correlating them with task performance \cite{vrzakova2020focused}.

%Use of machine learning concepts for collaboration problem-solving analysis and assessment is still relatively new in the Educational Data Mining community. Reilly \emph{et al.} used Coh-Metrix indices (a natural language processing tool to measure cohesion for written and spoken texts) to train machine learning models to classify co-located participant discourse in a multi-modal learning analytics study  \cite{reilly2019predicting}. The multi-modal dataset consisted of eye-tracking, physiological and motion sensing data. They analyzed the collaboration quality between novice programmers that were instructed to program a robot to solve a series of mazes. However, they studied only two collaborative states thereby making it a binary classification problem. Huang \emph{et al.} used an unsupervised machine learning approach to discover unproductive collaborative states for the same multi-modal dataset \cite{huang2019identifying}. For input features they computed different measures for each modality. Using an unsupervised approach they were able to identify a three-state solution that showed high correlation with task performance, collaboration quality and learning gain. Kang \emph{et al.} also used an unsupervised learning approach to study the collaborative problem-solving process of middle school students. They analyzed data collected using a computer-based learning environment of student groups playing a serious game \cite{kang2019collaborative}. They used \emph{KmL}, an R package useful for applying $k$-means clustering on longitudinal data \cite{genolini2011kml}. They too identified three different states using the proposed unsupervised method. In our paper we define five different group collaboration quality states in a supervised learning setup. The above studies discuss different ways to model positive collaboration between participants in a group. For Massive Open Online Courses (MOOCs), Alexandron \emph{et al.} proposed a technique to detect cheating in the form of unauthorized collaboration using machine learning classifiers trained on data of another form of cheating (copying using multiple accounts) \cite{alexandron2020towards}.

Guo and Barmaki used a deep-learning based object detection approach for analysis of pairs of students collaborating to locate and paint specific body muscles on each other \cite{guo2019collaboration}. They used a Mask R-CNN for detecting the students in the video recordings. They claim that close proximity of group participants and longer time taken to complete a task are indicators of good collaboration. However, they quantify participant proximity by the percentage of overlap between the student masks obtained using the Mask R-CNN. The amount of overlap can change dramatically across different view points. Also, collaboration need not necessarily be exhibited by groups that take a longer time to complete a task. In this paper, the deep-learning models are based off of the systematically designed multi-level conceptual model shown in Figure \ref{figure_workflow}. %The proposed approach utilizes features at lower levels of our conceptual model but we go well beyond these and also include higher level behavior analysis as well roles taken on by students to predict the overall group collaboration quality.

%We propose using Mixup augmentation, an over-sampling approach together with an ordinal cross-entropy loss function to better handle limited and imbalanced training data. Over-sampling techniques have been commonly used to make the different label categories to be approximately equal. SMOTE is one of the oldest and most widely cited over-sampling methods proposed by Chawla \emph{et al.} \cite{chawla2002smote}. The controlled variant of Mixup that we propose is very similar to their approach. However, ordinal loss functions have not received as much attention since the label space of most current classification problems of interest do not exhibit an ordered structure or relationship. We refer interested readers to the following papers that talk about ordinal loss functions for deep ordinal classification \cite{hou2016squared,beckham2017unimodal}. In this paper we propose a simple variant of the regular cross-entropy loss that takes into account the relative distance of the predicted samples from their true class label location.
